SwiftBrush v2: Make Your One-step Diffusion Model Better Than Its Teacher

In this paper, we aim to enhance the performance of SwiftBrush, a prominent one-step text-to-image diffusion model, to be competitive with its multi-step Stable Diffusion counterpart. Initially, we explore the quality-diversity trade-off between SwiftBrush and SD Turbo: the former excels in image diversity, while the latter excels in image quality. This observation motivates our proposed modifications in the training methodology, including better weight initialization and efficient LoRA training. Moreover, our introduction of a novel clamped CLIP loss enhances image-text alignment and results in improved image quality. Remarkably, by combining the weights of models trained with efficient LoRA and full training, we achieve a new state-of-the-art one-step diffusion model, achieving an FID of 8.14 and surpassing all GAN-based and multi-step Stable Diffusion models. The project page is available at https://swiftbrushv2.github.io.

==> tables/9-10-11.tex <==
\begin{table}
\centering
\begin{tabular}{l|ccccc|} 
\hline
Models & \multicolumn{1}{c}{FID$\downarrow$} & \space{} CLIP$\uparrow$ & IS$\uparrow$ & Precision$\uparrow$ & \space{} Recall$\uparrow$ \\ 
\hline
SD Turbo  & 16.10 & \textbf{0.33} & 40.22 & 0.65 & 0.35                  \\
SD 2.1    & 15.46 & 0.30 & 30.18 & 0.47 & 0.46                  \\
${\text{SwiftBrush}}_{\text{SD Turbo}}$ & \textbf{14.59} & 0.29 & 29.02 & 0.43 & 0.55                  \\ 
\hline
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} 
\end{tabular}
\end{table}

==> tables/exp.tex <==
\begin{figure}[t!]
    \centering
    \begin{minipage}{0.6\textwidth}
        \centering
        \scriptsize
        \setlength{\tabcolsep}{5pt}
        \caption{\textbf{HPSv2 comparisons} between our method and previous work. $^{\dag}$ denotes reported numbers, $^{\ddag}$ denotes our rerun based on provided GitHubs. Ours* indicates training with additional image regularization. \textbf{Bold} indicates the best, while \underline{underline} indicates the second best.}
        \begin{tabular}{lcccc}
        \toprule
        \textbf{Method} & \textbf{Anime}    & \textbf{Photo}    & \textbf{Concept Art} & \textbf{Painting} \\ 
        \midrule
        SDv2.1$\dag$    & \underline{27.48} & 26.89             & \underline{26.86}    & \textbf{27.46}    \\ 
        \midrule
        SD Turbo$\ddag$             & \textbf{27.98}    & \underline{27.59} & \textbf{27.16}       & \underline{27.19} \\
        InstaFlow$\dag$ & 25.98 & 26.32          & 25.79             & 25.93 \\
        BOOT$\dag$      & 25.29 & 25.16          & 24.40             & 24.61 \\
        SwiftBrush$\dag$         & 26.91 & 27.21          & 26.32             & 26.37 \\ 
        \midrule
        Ours            & 27.13 & 27.56          & 26.69             & 26.76 \\
        Ours*           & 27.25 & \textbf{27.62} & \underline{26.86} & 26.77 \\
        \bottomrule
        \end{tabular}
        \label{tab:hps_compare}
    \end{minipage}
    \hfill
    \begin{minipage}{0.35\textwidth}
        \centering
        \includegraphics[width=\linewidth]{assets/survey.pdf}
        \caption{\textbf{User survey}. We asked participants to compare the quality and diversity of images generated by the teacher model and our method across 30 random text prompts.}
        \label{fig:enter-label}
    \end{minipage}
\end{figure}

==> tables/pr_compare.tex <==
\begin{table}[]
\begin{tabular}{lcc}
\multicolumn{1}{c}{\textbf{Method}}           & \textbf{Precision} & \textbf{Recall}  \\ \hline
\textbf{SDv1.5 \cite{SD} \dag}                & TBU                & TBU              \\
\textbf{SDv2.1 \cite{SD} \dag}                & \underline{0.61}   & 0.41             \\
\textbf{SD Turbo \cite{SDTurbo} \dag}         & \textbf{0.65}      & 0.35             \\
\textbf{InstaFlow-0.9B \cite{InstaFlow} \dag} & 0.53               & 0.45             \\ \hline
\textbf{Ours}                                 & 0.55               & \textbf{0.53}    \\
\textbf{Ours w/ regularizers}                 & 0.57               & \underline{0.52}
\end{tabular}
\caption{Comparison in terms of precision and recall comparing with others methods on MS COCO-30k. For multi-step diffusion models, we use 25 denoising step, and use guidance scale of 3.0 for SDv1.5, and 4.5 for SDv2.1, the config used for our teacher model. $\dag$ Results are derived from public pretrained models.}
\label{tab:pr_compare}
\end{table}

==> tables/workcompare.tex <==
\begin{table}[]
\centering
\begin{tabular}{lcc}
\multicolumn{1}{c}{\textbf{Method}} & \textbf{FID}     & \textbf{CLIP}    \\ \hline
\textbf{StyleGAN-T \cite{sauer2023stylegan} \dag}            & 13.90            & N/A              \\
\textbf{GigaGAN \cite{kang2023scaling} \dag}               & 9.09             & N/A              \\ \hline
\textbf{SDv1.5 \cite{SD} \dag}                & 8.78             & N/A              \\
\textbf{SDv2.1 \cite{SD} \ddag}               & 12.26            & \underline{0.32} \\
\textbf{SD Turbo \cite{SDTurbo} \ddag}             & 16.10            & \textbf{0.33}    \\ \hline
\textbf{UFOGen \cite{ufo} \dag}                & 12.78            & N/A              \\
\textbf{MD-UFOGen \cite{mobilediffusion} \dag}             & 11.67            & N/A              \\
\textbf{HiPA \cite{HIPA} \dag}                  & 13.91            & 0.31             \\
\textbf{InstaFlow-0.9B \cite{InstaFlow} \ddag}       & 13.33            & 0.30             \\
\textbf{DMD \cite{DMD} \dag}                   & 11.49            & \underline{0.32} \\ \hline
\textbf{Ours}                       & \underline{8.77} & \underline{0.32} \\
\textbf{Ours w/ regularizers}       & \textbf{8.14}    & \underline{0.32}
\end{tabular}
\caption{Comparison of our works comparing with others methods on MS COCO-30k. For multi-step diffusion models, we use 25 denoising step, and use guidance scale of 3.0 for SDv1.5, and 4.5 for SDv2.1, which is the config used for our teacher model. $\dag$ Results are derived from original paper, $\ddag$ results are derived from public pretrained models.}
\label{tab:coco_compare}
\end{table}
